PropEM-L: Radio Propagation Environment Modeling and Learning for Communication-Aware Multi-Robot Exploration

Multi-robot exploration of complex, unknown environments benefits from the collaboration and cooperation offered by inter-robot communication. Accurate radio signal strength prediction enables communication-aware exploration. Models which ignore the effect of the environment on signal propagation or rely on a priori maps suffer in unknown, communication-restricted (e.g. subterranean) environments. In this work, we present Propagation Environment Modeling and Learning (PropEM-L), a framework which leverages real-time sensor-derived 3D geometric representations of an environment to extract information about line of sight between radios and attenuating walls/obstacles in order to accurately predict received signal strength (RSS). Our data-driven approach combines the strengths of well-known models of signal propagation phenomena (e.g. shadowing, reflection, diffraction) and machine learning, and can adapt online to new environments. We demonstrate the performance of PropEM-L on a six-robot team in a communication-restricted environment with subway-like, mine-like, and cave-like characteristics, constructed for the 2021 DARPA Subterranean Challenge. Our findings indicate that PropEM-L can improve signal strength prediction accuracy by up to 44% over a log-distance path loss model.

==> backup.tex <==
% timestamp                          0.552368
% receiver_x                        -0.024265
% receiver_y                        -0.268476
% receiver_z                         0.462850
% transmitter_x                      0.102855
% transmitter_y                     -0.164038
% transmitter_z                      0.107819
% freq_MHz                                NaN
% txpw_actual_dBm                    0.348800
% receiver_pose_time                 0.552966
% transmitter_pose_time              0.083096
% visible                           -0.805133
% distance                           0.802905
% obj_count_x                             NaN
% obj_count_y                        0.390378
% obj_count_z                        0.668349
% occupied_space_x                        NaN
% occupied_space_y                   0.404455
% occupied_space_z                   0.571948
% tx_spaciousness                    0.120704
% rx_spaciousness                    0.232377
% noise_level_dBm                    0.210054
% received_power_dBm                -0.998310
% measured_path_loss_dB              1.000000
% snr_dB                            -0.981281
% theoretical_udp_throughput_Mbps   -0.797305
% estimated_udp_throughput_Mbps     -0.799813
% loss_rate_percent                  0.647219
% total_air_time_percent            -0.037524
% total_data_rate_Mbps              -0.047361
% num_spatial_streams               -0.748713
% Name: measured_path_loss_dB, dtype: float64

% [2.07699888] 50.80314569711775
% timestamp                          0.407697
% receiver_x                        -0.072734
% receiver_y                        -0.140410
% receiver_z                         0.345737
% transmitter_x                      0.092202
% transmitter_y                     -0.175917
% transmitter_z                      0.042657
% freq_MHz                                NaN
% txpw_actual_dBm                    0.369692
% receiver_pose_time                 0.408242
% transmitter_pose_time              0.158528
% visible                           -0.658376
% distance                           0.620967
% obj_count_x                             NaN
% obj_count_y                        0.294178
% obj_count_z                        0.559297
% occupied_space_x                        NaN
% occupied_space_y                   0.299054
% occupied_space_z                   0.452630
% tx_spaciousness                    0.155041
% rx_spaciousness                    0.162614
% noise_level_dBm                    0.099766
% received_power_dBm                -0.882358
% measured_path_loss_dB              0.887586
% snr_dB                            -0.842191
% theoretical_udp_throughput_Mbps   -0.689470
% estimated_udp_throughput_Mbps     -0.677822
% loss_rate_percent                  0.653603
% total_air_time_percent            -0.130144
% total_data_rate_Mbps              -0.087460
% num_spatial_streams               -0.726774
% logdist                            0.694761
% simple_prediction                  0.694761
% extra_loss                         1.000000
% Name: extra_loss, dtype: float64

% min: 0.0
% max: 58.07
% mean: 6.48
% stddev: 5.3
% median: 5.54
% mse: 70.03

    
% features: ['distance', 'visible', 'occupied_space_y', 'occupied_space_z', 'obj_count_y', 'obj_count_z', 'tx_spaciousness', 'rx_spaciousness']
% labels: ['measured_path_loss_dB']
% batch size: 2048 epochs: 100
% 100 epochs
% average absolute error: 4.195775475436062
% mean squared error: 33.383316568620316

% with scaling
% features: ['distance', 'visible', 'occupied_space_y', 'occupied_space_z', 'obj_count_y', 'obj_count_z', 'tx_spaciousness', 'rx_spaciousness']
% labels: ['measured_path_loss_dB']
% batch size: 2048 epochs: 100
% 30 epochs
% average absolute error: 5.362360937320686
% mean squared error: 48.055165081921814


Which of these features are most correlated with SNR?
\begin{itemize}
    % \item timestamp 0.64
    % \item receiverz 0.63
    \item visible -0.81
    \item distance 0.85
    \item object count (in the xy plane) 0.70
    \item object count (in the xz plane) 0.47
    \item occupied space (in the xy plane) 0.62
    \item occupied space (in the xz plane) 0.53
\end{itemize}
% timestamp                          0.639258
% receiver_x                        -0.274976
% receiver_y                        -0.295437
% receiver_z                         0.634510
% transmitter_x                     -0.081850
% transmitter_y                      0.035374
% transmitter_z                      0.103100
% freq_MHz                                NaN
% txpw_actual_dBm                    0.064765
% receiver_pose_time                 0.639434
% transmitter_pose_time             -0.072292
% visible                           -0.806363
% distance                           0.848602
% obj_count_x                             NaN
% obj_count_y                        0.473984
% obj_count_z                        0.697996
% occupied_space_x                        NaN
% occupied_space_y                   0.530485
% occupied_space_z                   0.616892
% tx_spaciousness                   -0.058708
% rx_spaciousness                    0.203257
% noise_level_dBm                    0.117748
% received_power_dBm                -0.998585
% measured_path_loss_dB              1.000000
% snr_dB                            -0.986565
% theoretical_udp_throughput_Mbps   -0.686015
% estimated_udp_throughput_Mbps     -0.696155
% loss_rate_percent                 -0.074803
% total_air_time_percent             0.124789
% total_data_rate_Mbps               0.046783
% num_spatial_streams               -0.455809
% logdist                            0.949024
% simple_prediction                  0.949024
% extra_loss                         0.829276
% Name: measured_path_loss_dB, dtype: float64



\begin{itemize}
    % \item receiverz 0.54
    \item visible -0.67
    \item distance 0.60
    \item object count (in the xy plane) 0.57
    \item object count (in the xz plane) 0.39
    \item occupied space (in the xy plane) 0.52
    \item occupied space (in the xz plane) 0.47
\end{itemize}
% [2.01451356] 50.9272764498135
% timestamp                          0.431985
% receiver_x                        -0.334083
% receiver_y                        -0.219060
% receiver_z                         0.540498
% transmitter_x                     -0.229638
% transmitter_y                      0.036654
% transmitter_z                     -0.003126
% freq_MHz                                NaN
% txpw_actual_dBm                   -0.041743
% receiver_pose_time                 0.432224
% transmitter_pose_time              0.028115
% visible                           -0.668123
% distance                           0.602722
% obj_count_x                             NaN
% obj_count_y                        0.386398
% obj_count_z                        0.566117
% occupied_space_x                        NaN
% occupied_space_y                   0.474797
% occupied_space_z                   0.518793
% tx_spaciousness                    0.009180
% rx_spaciousness                    0.203460
% noise_level_dBm                    0.006811
% received_power_dBm                -0.855378
% measured_path_loss_dB              0.851419
% snr_dB                            -0.834355
% theoretical_udp_throughput_Mbps   -0.557044
% estimated_udp_throughput_Mbps     -0.546542
% loss_rate_percent                 -0.201769
% total_air_time_percent             0.011854
% total_data_rate_Mbps              -0.001067
% num_spatial_streams               -0.388541
% logdist                            0.642698
% simple_prediction                  0.642698
% extra_loss                         1.000000
% Name: extra_loss, dtype: float64

    \item Simple pathloss: Using only LOS links, the fitted simple pathloss model is [2.01, 50.93].
% min: 0.0
% max: 28.68
mean: 10.13
% stddev: 6.59
% median: 9.49
mse: 145.98

    \item Simple pathloss nLOS attenuation: best fit of dB/m attenuation 0.31, with max pathloss is 127.
% min: 0.0
% max: 40.03
mean: 6.34
% stddev: 4.61
% median: 5.54
mse: 61.45

The maximum error here is quite large, but the mean error is much better. The simple pathloss model predicts values over a range that only goes up to 106dB which is an underestimate of the worst case we see (127dB).

    \item Two linear regressions (one LOS and one nLOS): [2.01,50.93], [2.85,48.11]
    
    
        % Features = ['distance']
    % \begin{itemize}
    %     \item Learns a piece-wise linear function
    %     \item 70 epochs to convergence
    %     \item ('average absolute error:', 5.3642585744220925)
    % \end{itemize}
    
    % Features = ['distance','visible']
    % \begin{itemize}
    %     \item Learns two distinct piece-wise linear functions
    %     \item 100 epochs
    %     \item average absolute error: 5.059509640554801
    % \end{itemize}    
    
    % Features = ['distance','visible','occupied space z']
    % \begin{itemize}
    %     \item 100 epochs
    %     \item average absolute error: 4.654583269170285
    % \end{itemize}     
    
    % Features = ['distance','visible','occupied space z','occupied space y','obj count y','obj count z']
    % \begin{itemize}
    %     \item 100 epochs
    %     \item average absolute error: 4.198472029462277
    %     \item mean squared error: 34.150752559990494
    % \end{itemize}      

==> notes_from_Ali.tex <==
%\title{Networked Multi-Robot Exploration via Radio Propagation Modeling and Learning in Challenging Environments}
%\title{Networked Multi-Robot Exploration: Studying the Impact of Radio Propagation Modeling and Learning}
% \title{Communication-Aware Multi-Robot Exploration: An Experimental Study on Modeling and Learning of the Radio Propagation Environment}
% communication-aware multi-robot exploration: a study on modeling and learning of the radio propagation environment

% You will get a Paper-ID when submitting a pdf file to the conference system
% \author{Author Names Omitted for Anonymous Review. Paper-ID 46}

% \author{Lillian Clark$^{1}$, Jeffrey A. Edlund$^{2}$, Marc Sanchez Net$^{2}$, Tiago Stegun Vaquero$^{2}$, and Ali-akbar Agha-mohammadi$^{2}$% 
% \thanks{$^{1}$Clark is with the Ming Hsieh Department of Electrical and Computer Engineering, University of
% Southern California.
%         {\tt\small lilliamc@usc.edu}}%
% \thanks{$^{2}$Authors are with NASA Jet Propulsion Laboratory, California Institute of Technology.
%         {\tt\small \{jeffrey.a.edlund, marc.sanchez.net, tiago.stegun.vaquero, aliakbar.aghamohammadi\} @jpl.nasa.gov}}%
% }

% \author{\authorblockN{Lillian Clark}
% \authorblockA{Ming Hsieh Department of \\Electrical and Computer Engineering\\
% University of Southern California\\
% Email: lilliamc@usc.edu}
% \and
% \authorblockN{Jeffrey A. Edlund, Marc Sanchez Net, \\Tiago Stegun Vaquero, and Ali-akbar Agha-mohammadi}
% \authorblockA{NASA Jet Propulsion Laboratory\\
% California Institute of Technology\\
% Emails: \{jeffrey.a.edlund, marc.sanchez.net, \\tiago.stegun.vaquero, aliakbar.aghamohammadi\} @jpl.nasa.gov}
% }

% NeBula (few places)

% Chord
% Achord; IROS-Arxiv
% planetary cave (1-2): intro - Penny Boston - Jen Blank - Ali's scholar...
% Roadmap, MACIE
% lidar mapping: locus - lamp - lamp v2.0


% Deployable Mesh Network for Enabling Reliable Communication from within Subsurface Voids to the Planetary Surface
% MF Ginting, T Touma, J Edlund, A Buscicchio, K Otsu, A Aghamohammadi
% AGU Fall Meeting 2020	1	2020

% general missino/autonomy: 
% One Operator to Rule Them All: Human-Robot Interaction for Real-World and Analog Subsurface Exploration
% M Kaufmann, TS Vaquero, K Otsu, G Beltrame, A Agha-mohammadi
% Pasadena, CA: Jet Propulsion Laboratory, National Aeronautics and Space …
% Supervised Autonomy for Communication-degraded Subterranean Exploration by a Robot Team
% K Otsu, S Tepsuporn, R Thakker, TS Vaquero, JA Edlund, W Walsh, ...
% 2020 IEEE Aerospace Conference, 1-9


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

nebula (check) (check)
chord (check) (check)
achord (check) (check)
Boston (check) (check)
Blank (check) (check)
Locus (check) (check)
Lamp (check) (check)
deployable (check) (check)
ostu (check) (check)

==> notes_on_data.tex <==
sep18d, clean radio links
229918 rows × 36 columns

Correlation to measured path loss
* visible -0.84 *
* distance 0.86 *
* occupied_space 0.67 *
* maybe_occupied_space 0.71 *
* free_space 0.67 *
* unknown_space 0.62 *
tx_xwidth -0.21
tx_ywidth -0.29
tx_zwidth -0.17
rx_xwidth -0.1
rx_ywidth -0.36
rx_zwidth -0.26
* strict_visible -0.83 *
* strict_non_visible 0.82 *
* logdist 0.95 *

all_best_fit --- All data (fake links): 3.14, 47.3
simple_prediction --- General: 2.74, 47.50
two_line_prediction ---
LOS: 2.01, 50.83
nLOS (strict): 3.52, 33.31
heuristic_prediction ---
dB / m: 0.14058806526180917
max pathloss: 130.51502990722656

Correlation to loss beyond LOS pathloss
* visible -0.64 *
* distance 0.63 *
* occupied_space 0.55 *
* maybe_occupied_space 0.62 *
free_space 0.37
* unknown_space 0.55 *
tx_xwidth -0.13
tx_ywidth -0.18
tx_zwidth -0.05
rx_xwidth -0.11
rx_ywidth -0.29
rx_zwidth -0.14
* strict_visible -0.56 *
* strict_non_visible 0.56 *
* logdist 0.62 *

Including fake links
all_best_fit 5.51
simple_prediction 9.44
two_line_prediction 7.26
heuristic_prediction 8.22

Only real data
all_best_fit 7.11
simple_prediction 5.51
two_line_prediction 5.02
heuristic_prediction 5.06

Only strict LOS
all_best_fit 5.95
simple_prediction 5.18
two_line_prediction 4.49
heuristic_prediction 4.49

Only strict nLOS
all_best_fit 7.59
simple_prediction 5.63
two_line_prediction 5.23
heuristic_prediction 5.31


KEY TAKEAWAYS:
Log distance is very very correlated with measured pathloss, and LOS/nLOS is also very correlated. The classification of space is noticeably correlated, but the spaciousness features are not.

The best line of fit is pretty dramatically different for LOS and nLOS data.

The additional loss beyond a distance based model using the LOS fitted parameters is noticeably correlated with distance and LOS/nLOS.

On the data itself, the two line and heuristic models both perform well (mean error of 5dB). When we test these models on the data which include fake links, the two line model separates itself as the best.


TESTING ON COMP DATA: (These all include fake links, and are only the links we would try to predict, ie the receiver is a robot).

Day 1
all_best_fit 13.8
simple_prediction 16.31
two_line_prediction 17.0
heuristic_prediction 17.25

Day 2
all_best_fit 16.12
simple_prediction 18.85
two_line_prediction 30.28
heuristic_prediction 20.05

Day 3
all_best_fit 12.79
simple_prediction 13.44
two_line_prediction 24.86
heuristic_prediction 13.89

KEY TAKEAWAY:
None of these models port well to this new, more complex environment.

% Data from KY underground Sep 18 game 4
% \begin{itemize}
%     \item 1,305,836 datapoints
%     \item 36 columns (25 "features", 12 used for learning, 10 "labels", 1 used for learning, 1 "tag")
%     \item 13 dropped radios, 6 robots, 1 base station
%     \item 300 meters in each of the x and y directions
%     \item 80 minutes of data
% \end{itemize}

==> old.tex <==
% To take a closer look, we refitted the simple pathloss, two line, and heuristic models to the data from the competition and saw drastically different results (Table \ref{tab:different_envs}). \textcolor{red}{Why do the results differ so much from one day of competition to another? Map errors are probability a significant reason.}

% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c}
%         Parameter & Field test & Competition \\
%         \hline
%         $\eta$ & & \\
%         $PL(d_0)$ & & \\
%         $\eta^{LOS}$ & & \\
%         $PL(d_0)^{LOS}$ & & \\        
%         $\eta^{nLOS}$ & & \\
%         $PL(d_0)^{nLOS}$ & & \\     
%         dB/m & & \\
%     \end{tabular}
%     \caption{Key parameters which illustrate differences between the field test and competition environments.}
%     \label{tab:different_envs}
% \end{table}

% \section{Results}

% \begin{itemize}
%     \item qualitative difference between field test and competition data
%     \item summary of model performance
% \end{itemize}

% See spreadsheet for detailed summary of results. Overall the NN trained on distance, LOS/nLOS, and occupied space in the xy-plane performed the best with avg abs error of 11.54, 11.88, and 13.33 dB on the different competition days.

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{images/true_comp2.png}
%     \caption{3D map of the connectivity (ground truth). Note that measurements are shown to the nearest radio, and measurements taken before a radio was dropped may be outdated.}
%     \label{fig:true_comp2}
% \end{figure}

\begin{table}[]
    \centering
    \begin{tabular}{c|c}
        Feature & Correlation with signal attenuation \\
        \hline
        Log distance (m) & 0.95 \\
        Line of sight (y/n) & 0.83 \\
        Occupied voxels (number) & 0.67 \\
        Tx spaciousness (m) & 0.29 (y-direction) \\
        Rx spaciousness (m) & 0.36 (y-direction) \\
    \end{tabular}
    \caption{Correlation between features extracted from sparse point cloud data and measured signal strength attentuation.}
    \label{tab:feature_correlation}
\end{table}

% \begin{itemize}

%     % We train a two-layer NN for 100 epochs and vary the features it's fed.
    
%     \item NN: distance and strict visible -- MAE 5.43 dB
     
%     \item NN: distance and space classification -- MAE 5.04 dB
    
%     \item NN: distance and space classification and spaciousness -- MAE 3.46 dB


%     % Using distance, the NN learns a piece-wise linear function.
%     % Adding LOS/nLOS, the NN learned two distinct piece-wise linear functions and performance improves.
%     % Adding occupied space in the xy-plane (the most highly correlated), performance improves again.
%     % Adding occupied space in the xz-plane and object count estimations in the xy-plane and the xz-plane, performance improves again.
%     % Adding spaciousness doesn't change performance significantly.
%     % Scaling the distance and occupied space so that these feature values are on the same order of magnitude as the others hurts performance.
    
    
    
% \end{itemize}
   
% \subsection{Gaussian Processes}

% Time-allowing I will add to this section, but given the SubT Summit deadline coming up, I might try to finish the narrative with the current dataset and feature extraction and only the regression and NN methods.

% \begin{itemize}
%     \item exploring subterranean environment strains connectivity
%     \item predicting connectivity is useful for situational awareness and autonomy
%     \begin{itemize}
%         \item robot-to-robot (or robot-to-base) communication
%         \item source-seeking
%         \item autonomous deployment (nodes or pair-robots e.g. drone takeoff)
%         \item RSSI-based localization
%     \end{itemize}
%     \item we focus on SNR as high capacity links allow transferring images/science data
%     \item this research was used in the DARPA SubT challenge
% \end{itemize}

% However, it does not capture anything about whether the two are in a large cavernous space where the receiver is unlikely to receive bounced signals that interfere constructively, or a narrow corridor where reflections are likely. Thus in addition we use the 3D occupancy grid to consider the space immediately surrounding both the transmitter and receiver. We measure the width of free space in the x, y, and z directions around the radio to capture the \textit{spaciousness} of the environment.


% 10.99/12.47/11.89 dB on data from competition day 1/2/3, which is an improvement compared to 13.93/14.14/12.57 dB using the model trained offline. 

% The error over time of our online visibility model with $n=1$ is shown in Fig. \ref{fig:online}. At first, the testing error peaks above the training error because too few measurements are available, but as exploration continues both errors stabilize.

% Comp1: best case linear 11.95 dB
% Comp2: best case linear 12.93 dB
% Comp3: best case linear 11.96 dB

% Comp1: best case visibility 10.99 dB
% Comp2: best case visibility 12.47 dB
% Comp3: best case visibility 11.89 dB

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{images/visonline1b.png}
%     \caption{Linear regressions performed on LOS and nLOS links online every 60 seconds (day 1 of competition).}
%     \label{fig:online}
% \end{figure}

% \begin{itemize}
%     \item Regression: linear fit, LOS linear fit + nLOS linear fit, LOS linear fit + dB/m linear fit
%     % \item compare every X mins
%     \item Results: two lines online outperforms complex models trained offline
%     \item Discussion: Training more often improves average error (1 min is best). There is an optimal frequency to train to keep the maximum error low, as training too soon means weighing sparse data to heavily but training too infrequently means relying on the old model longer.
%     % \item TO DO: GP
% \end{itemize}

% \subsection{Online learning}


% Exploring expansive and unknown subterranean environments is a challenge multi-robot systems are well-suited for, with applications in lunar and planetary exploration \cite{vaquero2018approach}, and disaster mitigation \cite{murphy2009mobile}. The increased coverage and redundancy offered by a team of robots can improve exploration performance. Multi-robot teams benefit from the collaboration and cooperation offered by inter-robot communication \cite{yan2013survey}. However, these harsh environments are typically infrastructure-denied, meaning robots cannot rely on wireless access points for communication, and communication signals see significant degradation due to the scale of the environment, branch-like characteristics, and obstacles.



propose a  Propagation-Environment Model (PropEM) which uses a sensor-derived 3D geometric representation of the environment to infer its effect on signal attenuation.



X, a method for accurate signal strength modeling and prediction. The contributions and highlights of our work are:
\begin{enumerate}
    \item \ph{propose X} X combines the strengths of environment-aware attenuation models and data-driven  learning to achieve high-accuracy prediction. The attenuation models leverage sensor-derived point clouds and well-known models of signal propagation phenomena including free space path loss, shadowing due to obstacles, and multipath components.
    \item \ph{deploy X and show it's adaptable}
    \item \ph{use X}
\end{enumerate}

To enable multi-robot exploration in communication-restricted environments, we propose a method for accurate signal strength prediction. 

\ph{comparison and arch}
Leveraging well-known propagation models which account for free space path loss, reflection, and diffraction, we propose two approaches to learning: linear regression and neural networks.

\ph{Geometric-based attentiouation model (GAM)}
we propose GAM to construct Geometric-based attentiouation model. GAM extracts salient features (for radio signal propagation) from the 3D representation of the environment, constrcutred in real-time by robot's onboard sensors.

\ph{Geo-Radio data-driven modelling}
These features, combined with RSS measurements, inform learned models of signal attenuation.

Leveraging well-known propagation models which account for free space path loss, reflection, and diffraction, we propose two approaches to learning: linear regression and neural networks.


The key contributions of this work are:
\begin{enumerate}
    \item We propose a method for modeling line-of-sight obstructions and Fresnel zone clearance given sparse 3D point clouds.
    \item We present data-driven models which enable high-accuracy signal strength prediction to within a few decibels.
    \item We demonstrate how online learning allows these models to adapt to completely new environments.
    \item \ph{?? Adaptaion} We illustrate how RSS prediction can be used to generate signal strength maps for situational awareness and improved multi-robot autonomy.
    \item (an important contribuiont is .... we deploy the system)
\end{enumerate}

We evaluate the performance of our models using data from field tests in a limestone mine and during the DARPA Subterranean Challenge, and discuss how online learning can improve both signal strength prediction and our understanding of the material properties of the environment.

    % We consider data-driven approaches to radio signal strength prediction for a multi-robot system exploring communication-restricted subterranean environments. % 6
    % Rather than using models which ignore the effect of the environment on signal propagation or rely on \textit{a priori} maps, we leverage data available in real time from sensors on board the robots. During exploration, we use position estimates and 3D LiDAR point cloud data to extract information about line-of-sight between radios, and the presence of walls/obstacles which can cause attenuation, diffraction, and reflection. 
    % We develop several models, based on well-known signal propagation models and data-driven machine learning models, using data collected by a six-robot team in a limestone mine and compare their performance on data collected in a subterranean environment with subway-like, mine-like, and cave-like characteristics, constructed for the 2021 DARPA Subterranean Challenge. We demonstrate that the insight extracted from online-learning on LiDAR data can improve signal strength estimation by 44\% over a log-distance path loss model.
    
    
\ph{handling dynamic environments}
It is important to note that obstacles in the environment can be dynamic (e.g. the movement of scientists/supervisors who share the space, or the addition of barriers/tarps to section off geographic areas during operation). Thus our 3D model of the environment can change due to A) our changing understanding of the environment from visiting or revisiting and area and/or B) changes in the environment itself. 
% Through experimentation we determined that a log-likelihood of $X < l < Y$, which we classify as \textit{possibly occupied}, captures these dynamic obstacles as well as our uncertainty in areas which have only been visited briefly. 

% ``In computer graphics, a digital differential analyzer (DDA) is hardware or software used for interpolation of variables over an interval between start and end point. DDAs are used for rasterization of lines, triangles and polygons. They can be extended to non linear functions, such as perspective correct texture mapping, quadratic curves, and traversing voxels." 

% \textcolor{red}{Instead of x,y,z-spaciousness at transmitter and receiver, I could try to sample the width/height of the hallway - normal to the ray - every 5(?) meters along the ray from tx to rx and return the minimum cross-sectional area and maximum cross-sectional area?. To do: what tools exist for performing ray tracing (including absorptions and reflections) given an openvdb model?}



% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{images/feature_extraction.png}
%     \caption{Visualization of classifying space into free, occupied, and unknown space for obstacle thickness prediction.}
%     \label{fig:raytracing}
% \end{figure}
% \lillytodo{Smaller raytracing picture (with maybe occupied) -- or joint figure with fresnel zone too.}

% After cleaning up the data, the standard deviation on average for a given pair of transmitter and receiver locations is 0.52 dB for an average of 4 measurements each.
% , while the standard deviation on average at a given distance is 1.65 dB, and the standard deviation on average at a given distance rounded to the nearest meter is 5.77 dB.

% \textcolor{red}{How much stronger would this paper be another field test data set? ie the LA Subway}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{images/LOS_best_fit_edit.png}
%     \caption{Simple pathloss model learned via linear regression on LOS links.}
%     \label{fig:LOS_best_fit}
% \end{figure}

% Given our understanding of the physical characteristics of signal propagation, it is reasonable to also consider a model which uses not just visibility but the amount of free space/occupied space. Making the simplifying assumption that unknown space is the interior of obstacles and therefore occupied, 

% \begin{table}
%     \centering
%     \begin{tabular}{c|c|c|c}
%         Model & Day 1 & Day 2 & Day 3 \\
%         \hline \hline
%         Simple path loss & 15.87 & 15.37 & 13.0 \\
%         Visibility & \textbf{13.93} & \textbf{14.14} & \textbf{12.57} \\
%         Heuristic & 14.12 & 14.55 & 12.88 \\
%         \hline 
%         Two-Ray & 17.59 & 17.86 & 16.57 \\
%         Knife-edge & \textbf{13.54} & \textbf{14.69} & \textbf{13.36} \\
%         Reflection-Diffraction & 13.93 & 15.45 & 14.11 \\
%         \hline 
%         NN Model 1 & 12.63 & 13.42 & 12.03 \\
%         NN Model 2 & 11.87 & \textbf{12.70} & \textbf{11.21} \\
%         NN Model 3 & 13.00 & 13.56 & 12.58 \\
%         NN Model 4 & 12.64 & 14.99 & 12.43 \\
%         NN Model 5 & \textbf{11.42} & 12.95 & 11.70 \\
%     \end{tabular}
%     \caption{Mean absolute error (dB) for each model during each run of the DARPA SubT Challenge.}
%     \label{tab:results}
% \end{table}

% comp1 LOS (1.83, 48.71) nLOS (5.11, 20.17) db/m 0.43 -- clean2
% comp2 LOS (1.59, 46.83) nLOS (4.98, 20.81) db/m 0.63
% comp3 LOS (1.94, 42.15) nLOS (4.43, 27.71) dB/m 0.66


% Comparing the fitted LOS and nLOS linear models to the competition data highlights that the nLOS linear model is very different. This is likely because the materials making up the environment were very different and this isn't captured in the model (the only information we have available is the thickness). Through online learning, we can refine our understanding of the material/the attenuation per occupied meter (on average for the new environment).


\lillytodo{focus on comm-aware exploration}
We have evaluated our prediction models based on their ability to accurately predict the strength of a signal received by a robot from one or multiple nearby radios. This knowledge is useful for several aspects of situational awareness and autonomy, and may be crucial for human-autonomy teaming. 
Fig. \ref{fig:ssm_grid} shows a heatmap of the predicted signal strength for the competition environment, overlaid on the 3D point cloud data, demonstrating the capability to predict for an arbitrary location the received strength of a signal which was transmitted by any of the known stationary radios, and visualize this data in a signal strength map. Beyond capturing areas we have already explored, this predictive signal strength map can be used to encourage robots to explore new areas which are expected to offer connectivity, allowing timely data transfer of new information.

% \ph{NN models}
Each NN takes a subset of the features which PropEM outputs, as described below:
\begin{itemize}
    \item \textbf{NN-vis} uses logarithmic distance and LOS, which is broken into two boolean input features: \textit{strictly visible} indicates all the voxels between the transmitter and receiver are free; \textit{strictly not visible} indicates there is at least one occupied voxel.
    % NN-vis converged in 40 epochs.
    \item \textbf{NN-vox} uses logarithmic distance and the number of occupied, maybe occupied, free, and unknown voxels. 
    % NN-vox converged in 66 epochs.
    \item \textbf{NN-ref} uses logarithmic distance and reflection loss.
    % , and did not converge.
    \item \textbf{NN-diff} uses logarithmic distance and diffraction loss.
    % , and converged in 5 epochs.
    \item \textbf{NN-all} uses the combined features of models 2, 3, and 4.
    % , and converged in 90 epochs.
\end{itemize}
